GuideTWSI: A Diverse Tactile Walking Surface Indicator Dataset from Synthetic and Real-World Images for Blind and Low-Vision Navigation

Tactile Walking Surface Indicators (TWSIs) are safety-critical landmarks that blind and low-vision (BLV) pedestrians use to locate crossings and hazard zones. From our observation sessions with BLV guide dog handlers, trainers, and an O&M specialist, we confirmed the critical importance of reliable and accurate TWSI segmentation for navigation assistance of BLV individuals. Achieving such reliability requires large-scale annotated data. However, TWSIs are severely underrepresented in existing urban perception datasets, and even existing dedicated paving datasets are limited: they lack robot-relevant viewpoints (e.g., egocentric or top-down) and are geographically biased toward East Asian directional bars - raised parallel strips used for continuous guidance along sidewalks. This narrow focus overlooks truncated domes - rows of round bumps used primarily in North America and Europe as detectable warnings at curbs, crossings, and platform edges. As a result, models trained only on bar-centric data struggle to generalize to dome-based warnings, leading to missed detections and false stops in safety-critical environments.

==> old_text.tex <==


% \hc{Add human study in both abstract and introduction}

% Tactile paving provides vital environmental cues (e.g., crossing points, hazard warnings) for blind and low-vision (BLV) pedestrians, yet remains critically underrepresented in existing urban perception datasets. This limits the ability of autonomous systems to reason about the semantics of sidewalks with diverse materials, textures, and layouts. We introduce a comprehensive framework for tactile paving segmentation with three core contributions: (1) a photorealistic synthetic data generation pipeline that simulates multiple types of tactile paving under varied surface conditions and viewpoints, producing over 10K samples; (2) a diverse, large-scale dataset combining open-source annotations and real-world images collected via a quadruped robot; and (3) extensive evaluations of state-of-the-art segmentation models showing \hc{(mIoU ↑X\%)}, including real-world deployment on a mobility-assistive guide-dog robot. Our ablation studies show that training with additional synthetic data significantly improves segmentation robustness across domains. Furthermore, we demonstrate that enhanced segmentation leads to substantial gains in downstream robot decision-making, notably in accurate stop inference at tactile zones. Dataset, code, pretrained model checkpoints, and videos are released at: \href{https://github.com/DARoSLab/NavAble.git}{https://github.com/DARoSLab/NavAble.git}.



% While tactile sensors are inexpensive, they only activate upon direct contact, which is too late for safe stopping. Guide robots that rely on vision to anticipate pavings and deliver the life-saving “stop and decide” signal in advance.


% To overcome these limitations, we propose **SToP-15K**, a photorealistic synthetic dataset of tactile pavings generated with a scalable Unreal Engine 4 pipeline (NDDS~\cite{to2018ndds}, AirSim~\cite{airsim2017fsr}) that models diverse paving types, materials, lighting, weather, and robot viewpoints. Integrated with curated open-source annotations and real-world images collected using a quadruped robot, SToP-15K establishes the largest and most diverse dataset for tactile paving segmentation.  




% To overcome these limitations, we propose **SToP-15K**, a photorealistic synthetic dataset of tactile pavings generated with a scalable Unreal Engine 4 pipeline (NDDS~\cite{to2018ndds}, AirSim~\cite{airsim2017fsr}) that models diverse paving types, materials, lighting, weather, and robot viewpoints. Integrated with curated open-source annotations and real-world images collected using a quadruped robot, SToP-15K establishes the largest and most diverse dataset for tactile paving segmentation.  


% Tactile pavings provide vital environmental cues -- such as pedestrian crossing points, platform edges, hazard zones -- for blind and low-vision (BLV) pedestrians. These textured ground indicators, typically composed of truncated domes and directional bars, offer multisensory feedback through touch, sight, and sound. Despite their critical role in accessible urban design and regulation (e.g., ADA, California Title 24, and AASHTO M 333-16), tactile pavings remain severely underrepresented in existing urban perception datasets. This limits the ability of autonomous mobility assistive systems to understand sidewalk semantics across diverse materials, layouts, and lighting conditions.





% Tactile pavings are critical components of accessible urban design, providing environmental cues at crossings, platform edges, and hazard zones for blind and low-vision (BLV) pedestrians. These textured ground indicators, typically composed of truncated domes and directional bars, offer multisensory feedback through touch, sight, and sound, and are codified in regulations such as the ADA, California Title 24, and AASHTO M 333-16. For BLV travelers, tactile pavings are safety-critical landmarks: cane users detect them directly through hand–cane contact, while guide dogs are trained to stop at them so that handlers can probe the ground with a foot. 

% Tactile pavings are foundational elements of accessible urban infrastructure, marking crossings, transit edges, and hazard zones for blind and low-vision (BLV) pedestrians. These textured surfaces—typically truncated domes or directional bars—provide multisensory feedback through touch, sound, and sight, and are codified in accessibility regulations (e.g., ADA, California Title 24, and AASHTO M 333-16). For BLV travelers, they serve as safety-critical landmarks: cane users detect them directly through hand–cane contact, while guide dogs are trained to stop at them so that handlers can confirm the boundary with a foot.  

% Yet, our observation sessions with a guide dog handler, trainer, and orientation \& mobility (O\&M) specialist revealed that tactile paving detection is often unreliable in practice. Pavings may be worn, misaligned, or inconsistently installed, and even well-trained guide dogs sometimes stop before or after the landmark, leaving travelers uncertain about boundaries. These insights highlight both the importance and fragility of tactile pavings as decision cues. For affordable guide robots, the challenge is sharper: without tactile sensing, they must provide the life-saving *“stop and decide”* signal purely through visual perception, requiring highly reliable recognition.  

% Unfortunately, tactile pavings remain severely underrepresented in existing urban perception datasets, limiting the ability of autonomous mobility aids to reason about sidewalk semantics across diverse materials, layouts, and lighting conditions. Even dedicated tactile paving datasets are insufficient: they lack robot-relevant viewpoints (e.g., egocentric or top-down), are geographically biased toward East Asian directional bars, and underrepresent U.S.-style truncated domes that dominate high-stakes zones such as curb ramps and transit edges. As a result, models trained on these limited distributions struggle to generalize, risking missed detections and false stops in safety-critical environments.  







% \dhk{This paragraph seems odd. Real-world data is gained for real-world deployment? }
% For real-world deployment, we collected a real-world tactile paving dataset with a quadruped for guide dog robot applications. We further deployed the perception model on the real-robot and performed extensive tactile paving stopping demonstrations at various areas in rural, suburban, and urban areas. to test task-specific semantic segmentation - guide dog robot perception for tactile paving segmentation





%% HC
% Tactile paving (raised ground textures like truncated domes and ridged bars) provides vital cues for blind and low-vision (BLV) pedestrians. These patterns -- mandated by accessibility standards (e.g., ADA, California Title 24, and AASHTO M 333-16) -- alert BLV travelers to street crossings, platform edges, and other hazards. Despite their critical role in accessible urban design, tactile pavings are severely underrepresented in existing vision datasets. For example, SideGuide~\cite{park2020sideguide}, Tenji10K~\cite{takano2024tactile}, and TP~\cite{zhang2024grfb} dataset provide valuable sidewalk or paving images, but they are geographically biased toward East Asia (Japanese “tenji” blocks and aligned bars) and lack the U.S.-style truncated domes found on curb ramps and transit platforms. Moreover, existing images are typically captured under limited viewpoints (e.g., human eye-level) and lighting, limiting the robustness of models to understand sidewalk semantics across diverse conditions when deployed on autonomous mobility assistive robots.


% These gaps have practical consequences. A failure to detect tactile pavings directly endangers navigation safety, as the robot may miss the stop cue at a curb ramp or crossing. Unlike semantic errors in car perception (which may be smoothed by map priors or sensor redundancy), errors in assistive navigation directly compromise the safety of a BLV handler. Robust tactile paving perception is thus an unsolved bottleneck for real-world deployment of vision-based guide robots~\cite{takagi2025field, cai2024navigating, hwang2024towards}. 

% %%
% To overcome these gaps, we introduce a photorealistic synthetic data pipeline for tactile paving segmentation. Using Unreal Engine 4 (UE4) and AirSim, we procedurally generate diverse street scenes with diverse tactile pavings under varied materials, colors, lighting, and camera angles. Our pipeline automatically produces precise ground-truth labels (masks, boxes, depth) for each synthetic image. We generated over 10,000 labeled images of tactile pavement to augment training of state-of-the-art segmentation models. In parallel, we collected a real-world tactile paving dataset (“TactileReal”) with a quadruped guide-dog robot to reflect practical deployment scenarios. We then fine-tune modern segmentation architectures (e.g., SAMv2.1, YOLO-Seg) on combined real and synthetic data.



% As a result, models trained on them often fail to generalize, leading to missed detections or false stops hindering reliable stopping at tactile pavings for sidewalk robots~\cite{takagi2025field,cai2024navigating,hwang2024towards} and delivery platforms - no real-world demonstrations of robots stopping at tactile pavings have been shown. 

% -- high-stakes decision zones where precise segmentation is essential for downstream actions such as safe stopping. Yet current datasets rarely cover these conditions and lack diversity in viewpoints (e.g., egocentric, top-down) and environmental factors (lighting, weather, material). This limits the robustness and generalization of models when deployed on autonomous sidewalk platforms such as guide robots~\cite{takagi2025field,cai2024navigating,hwang2024towards} and delivery bots.


% Dedicated tactile paving datasets have begun to address this gap, including SideGuide~\cite{park2020sideguide}, Tenji10K~\cite{takano2024tactile}, and TP~\cite{zhang2024grfb}. However, they exhibit three major limitations: (i) geographic bias toward East Asia, where directional bars dominate, while U.S. infrastructure relies on truncated domes at high-stakes decision zones such as curb ramps and transit edges; (ii) lack of robot-relevant viewpoints, such as egocentric and top-down, which stakeholders (e.g., guide-dog trainers) emphasize are critical for stopping exactly “on the bump dots”; and (iii) limited diversity in conditions such as material, weather, and lighting, restricting model robustness in real-world deployment. As a result, current models often fail to generalize, risking missed detections or false stops in safety-critical environments.



% Dedicated tactile paving datasets have begun to address this gap, including SideGuide~\cite{park2020sideguide}, Tenji10K~\cite{takano2024tactile}, and TP~\cite{zhang2024grfb}. However, they exhibit three major limitations: (i) geographic bias toward East Asia, where directional bars dominate, while U.S. infrastructure relies on truncated domes at high-stakes decision zones such as curb ramps and transit edges; (ii) lack of robot-relevant viewpoints, such as egocentric and top-down, which stakeholders (e.g., guide-dog trainers) emphasize are critical for stopping exactly “on the bump dots”; and (iii) limited diversity in conditions such as material, weather, and lighting, restricting model robustness in real-world deployment. As a result, current models often fail to generalize, risking missed detections or false stops in safety-critical environments.  



% \dhk{We can explain with the guide-dog trainers' comments: they said that it is important to train a dog to stop at bump dots - tactile pavings serve as a critical landmark for BLV. Also, a robot stops at the right above the bump dots - this may give a justification for the chin camera (top-down view) }




% To overcome these limitations, we develop a customizable synthetic data generation framework tailored for tactile paving segmentation. We generate high-diversity data spanning multiple paving types, colors under different lighting conditions, and viewpoints, using Unreal Engine 4 (UE4). Combined with AirSim~\cite{airsim2017fsr} for automated annotation, our framework offers photorealistic rendering and ground-truth labels.  We generated a large-scale synthetic tactile paving dataset, \emph{SToP-15K}, to fine-tune state-of-the-art segmentation models. [Details on synthetic data (stop-15k), curated data, and robot data.]

% \dhk{You may want to add some explanations about this dataset.} \hc{details on curated real data and robot-collected data }

% For ablation studies, we curated open-source tactile paving datasets and augmented our synthetic data to evaluate the effectiveness of our synthetic data. We further collected real-world images using a quadruped robot and manually annotated them to analyze both quantitative performance and 

% [more details of score put scores in X,Y,Z for now]
% qualitative downstream behavior -- reliable stopping at tactile pavings. This dataset was used to quantitatively evaluate our benchmark and fine-tuned models. To our knowledge, this is the first work to achieve reliable tactile paving–based stopping across diverse, previously unseen environments, deployed on a real guide robot.

